Microwave calibration of qubit drive line components at millikelvin temperatures

Systematic errors in qubit state preparation arise due to non-idealities in the qubit control lines such as impedance mismatch. Using a data-based methodology of short-open-load calibration at a temperature of 30 mK, we report calibrated 1-port scattering parameter data of individual qubit drive line components. At 5~GHz, cryogenic return losses of a 20-dB-attenuator, 10-dB-attenuator, a 230-mm-long 0.86-mm silver-plated cupronickel coaxial cable, and a 230-mm-long 0.86-mm NbTi coaxial cable were found to be 35$^{+3}_{-2}$ dB, 33$^{+3}_{-2}$ dB, 34$^{+3}_{-2}$ dB, and 29$^{+2}_{-1}$ dB respectively. For the same frequency, we also extract cryogenic insertion losses of 0.99$^{+0.04}_{-0.04}$ dB and 0.02$^{+0.04}_{-0.04}$ dB for the coaxial cables. We interpret the results using a master equation simulation of all XY gates performed on a single qubit. For example, we simulate a sequence of two 5 ns gate pulses (X & Y) through a 2-element Fabry-P\'erot cavity with 276-mm path length directly preceding the qubit, and establish that the return loss of its reflective elements must be >9.7 dB (> 14.7 dB) to obtain 99.9 % (99.99 %) gate fidelity.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
